Polarization Holes as an Indicator of Magnetic Field-Angular Momentum Alignment I. Initial Tests

The formation of protostellar disks is still a mystery, largely due to the difficulties in observations that can constrain theories. For example, the 3D alignment between the rotation of the disk and the magnetic fields (B-fields) in the formation environment is critical in some models, but so far impossible to observe. Here, we study the possibility of probing the alignment between B-field and disk rotation using ``polarization holes'' (PHs). PHs are widely observed and are caused by unresolved B-field structures. With ideal magnetohydrodynamic (MHD) simulations, we demonstrate that different initial alignments between B-field and angular momentum (AM) can result in B-field structures that are distinct enough to produce distinguishable PHs. Thus PHs can potentially serve as probes for alignments between B-field and AM in disk formation.

==> tabs/pred_snap32.tex <==
\begin{tabular}{ccccc}
\toprule
&$(\ell, 22.5^\circ, 45^\circ)$&$(\ell, 45^\circ, 45^\circ)$&$(\ell, 45^\circ, 90^\circ)$&$(\ell, 67.5^\circ, 90^\circ)$\tabularnewline
\midrule
$\ell=0^\circ$&$(90^\circ, 22.5^\circ, 0^\circ)$&$(0^\circ, 45^\circ, 0^\circ)$&$(0^\circ, 22.5^\circ, 0^\circ)$&$(0^\circ, 67.5^\circ, 0^\circ)$\tabularnewline
$\ell=90^\circ$&$(90^\circ, 22.5^\circ, 0^\circ)$&$(90^\circ, 45^\circ, 0^\circ)$&$(90^\circ, 45^\circ, 0^\circ)$&$(90^\circ, 67.5^\circ, 0^\circ)$\tabularnewline
\bottomrule
\end{tabular}


==> tabs/pred_snap33.tex <==
\begin{tabular}{ccccc}
\toprule
&$(\ell, 22.5^\circ, 45^\circ)$&$(\ell, 45^\circ, 45^\circ)$&$(\ell, 45^\circ, 90^\circ)$&$(\ell, 67.5^\circ, 90^\circ)$\tabularnewline
\midrule
$\ell=0^\circ$&$(0^\circ, 45^\circ, 0^\circ)$&$(0^\circ, 45^\circ, 0^\circ)$&$(0^\circ, 45^\circ, 0^\circ)$&$(0^\circ, 67.5^\circ, 0^\circ)$\tabularnewline
$\ell=90^\circ$&$(90^\circ, 22.5^\circ, 0^\circ)$&$(90^\circ, 45^\circ, 0^\circ)$&$(90^\circ, 45^\circ, 0^\circ)$&$(90^\circ, 67.5^\circ, 0^\circ)$\tabularnewline
\bottomrule
\end{tabular}


==> tabs/pred_snap34.tex <==
\begin{tabular}{ccccc}
\toprule
&$(\ell, 22.5^\circ, 45^\circ)$&$(\ell, 45^\circ, 45^\circ)$&$(\ell, 45^\circ, 90^\circ)$&$(\ell, 67.5^\circ, 90^\circ)$\tabularnewline
\midrule
$\ell=0^\circ$&$(0^\circ, 22.5^\circ, 0^\circ)$&$(0^\circ, 45^\circ, 0^\circ)$&$(0^\circ, 45^\circ, 0^\circ)$&$(0^\circ, 67.5^\circ, 0^\circ)$\tabularnewline
$\ell=90^\circ$&$(90^\circ, 22.5^\circ, 0^\circ)$&$(90^\circ, 45^\circ, 0^\circ)$&$(90^\circ, 45^\circ, 0^\circ)$&$(90^\circ, 67.5^\circ, 0^\circ)$\tabularnewline
\bottomrule
\end{tabular}

